Language-Grounded Dynamic Scene Graphs for Interactive Object Search with Mobile Manipulation

To fully leverage the capabilities of mobile manipulation robots, it is imperative that they are able to autonomously execute long-horizon tasks in large unexplored environments. While large language models (LLMs) have shown emergent reasoning skills on arbitrary tasks, existing work primarily concentrates on explored environments, typically focusing on either navigation or manipulation tasks in isolation. In this work, we propose MoMa-LLM, a novel approach that grounds language models within structured representations derived from open-vocabulary scene graphs, dynamically updated as the environment is explored. We tightly interleave these representations with an object-centric action space. Given object detections, the resulting approach is zero-shot, open-vocabulary, and readily extendable to a spectrum of mobile manipulation and household robotic tasks. We demonstrate the effectiveness of MoMa-LLM in a novel semantic interactive search task in large realistic indoor environments. In extensive experiments in both simulation and the real world, we show substantially improved search efficiency compared to conventional baselines and state-of-the-art approaches, as well as its applicability to more abstract tasks. We make the code publicly available at http://moma-llm.cs.uni-freiburg.de.

==> figures/tex-figures/OLD/auc_curve.tex <==
\setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{1}
\begin{figure}[t]
	\centering
	\resizebox{\linewidth}{!}{%
 \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip,angle =0,valign=c]{figures/raw/auc_curve.png}}
	% \vspace{-0.2cm}
     \caption{Search Efficiency Curve in Simulation.}
  	\label{fig:auc}
   \vspace{-0.3cm}
\end{figure} 
\setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1}

==> tables/analysis.tex <==
    \begin{table}
        \centering
        \caption{Analysis of the different model behaviors. }
        \label{tab:analysis}
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|YYY}
          \toprule
            Model & \# Object Interactions & Distance Travelled & Infeasible Actions\\
          \midrule
            Random               & 7.0 & 42.4 & --\\
            Greedy               & 8.6 & 24.7 & --\\
            Random w/ door-prior & 9.3 & 25.7 & --\\
            Greedy w/ door-prior & 9.0 & 25.0 & --\\
            \midrule
            ESC                  & 5.8 & 28.2 & --\\
            HIMOS                & 5.3 & 43.2 & --\\
            \midrule
            Unstructured LLM     & 3.9 & 19.2 & 0.51 \\
            \ours{}              & 4.2 & 19.2 & 0.35 \\
          \bottomrule
        \end{tabularx}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Average over all episodes (including failures). Distance travelled in meters. Infeasible Actions is the average number of steps in which the LLM produces an action that could not be executed.
         \end{tablenotes}
       \end{threeparttable}
    \end{table}

==> tables/prompt_ablations.tex <==
    \begin{table}
        \scriptsize
        \setlength{\tabcolsep}{4pt}
        \centering
        \caption{Prompt Ablations}\label{tab:prompt_ablations}
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|YYY|YYY}
          \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{SR} & \multirow{2}{*}{SPL} & \multirow{2}{*}{AUC-E} & Object & Distance & Infeasible\\
             &  &  &  & Interactions & Traveled & Actions\\
            \midrule
            Unstructured LLM (w/ action history and frontiers)   & 86.3 & 59.4 & 77.6 & \underline{3.6} & 18.5 & 0.41 \\
            \midrule
            Structured Room-Object encoding w/o history, w/o frontiers & 76.0 & 55.8 & 69.6 & 3.9 & \underline{13.7} & 0.85 \\
            Structured Room-Object encoding + room-history, w/o frontiers & 79.4 & 54.9 & 72.4 & 4.2 & 15.5 & 0.94 \\
            Structured Room-Object encoding + action-history, w/o frontiers & 79.4 & 55.0 & 72.2 & 4.3 & 15.6 & 0.91 \\
            Structured Room-Object encoding w/o history w/ frontiers & 94.9 & \underline{63.0} & 84.1 & \underline{3.6} & 17.1 & 0.26 \\
            Structured Room-Object encoding + room-history + frontiers & \underline{97.1} & \underline{63.0} & \underline{86.6} & 3.8 & 17.8 & 0.28 \\
            \ours{} w/o distances and nearby objects & \underline{97.1} & 61.5 & 86.4 & 3.8 & 18.9 & 0.24 \\
            \midrule
            \ours{} (ours)           & \textbf{97.7} & \textbf{63.6} & \underline{87.2} & 3.9 & 18.2 & \underline{0.19} \\
            \midrule
            \ours{} w/ Hydra & 92.0 & 61.9 & 84.3 & \textbf{2.7} & \textbf{12.9} & \textbf{0.06}\\
          \bottomrule
        \end{tabularx}
        \vspace{-0.cm}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Best and second best highlighted in bold and underline. Object interactions, distance travelled and infeasible actions averaged over all episodes - including early terminated failures. Infeasible Actions: average number of steps the LLM produced an action that could not be executed, resulting in re-planning with continued conversation (cf. Sec. IV-C.4).
         \end{tablenotes}
       \end{threeparttable}
       \vspace{-0.3cm}
    \end{table}
